Pareto-Optimal Learning from Preferences with Hidden Context

Ensuring AI models align with human values is essential for their safety and functionality. Reinforcement learning from human feedback (RLHF) leverages human preferences to achieve this alignment. However, when preferences are sourced from diverse populations, point estimates of reward can result in suboptimal performance or be unfair to specific groups. We propose Pareto Optimal Preference Learning (POPL), which enables pluralistic alignment by framing discrepant group preferences as objectives with potential trade-offs, aiming for policies that are Pareto-optimal on the preference dataset. POPL utilizes lexicase selection, an iterative process that selects diverse and Pareto-optimal solutions. Our theoretical and empirical evaluations demonstrate that POPL surpasses baseline methods in learning sets of reward functions and policies, effectively catering to distinct groups without access to group numbers or membership labels. We verify the performance of POPL on a stateless preference learning setting, a Minigrid RL domain, Metaworld robotics benchmarks, as well as large language model (LLM) fine-tuning. We illustrate that POPL can also serve as a foundation for techniques optimizing specific notions of group fairness, ensuring safe and equitable AI model alignment.

==> images/synthetic_experiments/heatmap.tex <==
\begin{figure}[t]
    \centering
    % Row label z=0 (You might need to adjust positioning)
    \begin{minipage}{.05\textwidth}
        \centering
        \rotatebox{90}{\Large $z=0$}
    \end{minipage}
    % First row of images 
    \begin{minipage}{.9\textwidth}
        \begin{subfigure}{.33\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/synthetic_experiments/heatmaps/b_rex_passes_1_bradley-terry_1000_0.0.png}
            %\caption*{B-Rex}
        \end{subfigure}%
        \begin{subfigure}{.33\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/synthetic_experiments/heatmaps/lexicase_passes_1_1000_0.0.png}
            %\caption*{Lexicase}
        \end{subfigure}%
        \begin{subfigure}{.33\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/synthetic_experiments/heatmaps/b_rex_passes_1_lexicase_1000_0.0.png}
            %\caption*{LexicaseMCMC}
        \end{subfigure}
    \end{minipage}
    
    \vspace{5mm} % Provides a bit of vertical space between the rows
    
    % Row label z=1 (You might need to adjust positioning)
    \begin{minipage}{.05\textwidth}
        \centering
        \rotatebox{90}{\Large $z=1$}
    \end{minipage}
    % Second row of images
    \begin{minipage}{.9\textwidth}
        \begin{subfigure}{.33\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/synthetic_experiments/heatmaps/b_rex_passes_2_bradley-terry_1000_0.0.png}
            \caption*{B-Rex}
        \end{subfigure}%
        \begin{subfigure}{.33\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/synthetic_experiments/heatmaps/lexicase_passes_2_1000_0.0.png}
            \caption*{Lexicase}
        \end{subfigure}%
        \begin{subfigure}{.33\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/synthetic_experiments/heatmaps/b_rex_passes_2_lexicase_1000_0.0.png}
            \caption*{Lexicase MCMC}
        \end{subfigure}
    \end{minipage}
    \caption{Preference Pass Matrix with respect to two hidden context classes $z=0$ and $z=1$ for the distribution produced by all three reward inference methods. For each pair of the 100 states that we interpolate between $[0, 1]$, we display the number of reward functions in the distribution that pass that preference. Note that the Population based approach maintains a relatively small population size of 100, while the MCMC based approaches maintain the whole chain of size 10,000.}
    \label{fig:heatmap}
\end{figure}
